A self-monitoring precision calibration light source for large-volume neutrino telescopes

With the rise of neutrino astronomy using large-volume detector arrays, calibration improvements of optical media and photosensors have emerged as significant means to reduce detector systematics. To improve understanding of the detector volume and its instrumentation, we developed an absolutely-calibrated, self-monitoring, isotropic, nanosecond, high-intensity calibration light source called "Precision Optical Calibration Module" (POCAM). This now third iteration of the instrument was developed for an application in the IceCube Upgrade but, with a modular instrument communications and synchronization backend, can provide a calibration light source standard for any large-volume photodetector array. This work summarizes the functional principle of the POCAM and all related device characteristics as well as its precision calibration procedure. The latter provides fingerprint-characterized instruments with knowledge on absolute and relative behavior of the emitted light pulses as well as their temperature dependencies.

==> dump.tex <==
%
\begin{figure}[h!]
	\centering
    \begin{subfigure}[c]{0.9\textwidth}
	    \includegraphics[width=0.9\textwidth]{paper-intensity.pdf}
	    \caption{POCAM light pulser linearity. The figure shows the normalized intensity of all light pulse drivers with respect to applied bias voltage for the default $405\,$nm LED/LD at room temperature. All drivers show linear behaviour over most of their dynamic range.}
	    \label{fig:pulser-linearity}
	\end{subfigure}\vspace{1cm}
	%
	\begin{subfigure}[c]{0.9\textwidth}
	    \includegraphics[width=0.9\textwidth]{paper-timeprofile.pdf}
	    \caption{POCAM light pulser time profiles. The figure shows the normalized time profiles of all light pulse drivers with respect to minimal-working (top) and maximal (bottom) applied bias voltage for the default $405\,$nm LED/LD at room temperature. As expected, with larger currents driving the pulses at higher voltages, the light pulses gain in width.}
	    \label{fig:pulser-timing}
	\end{subfigure}
\end{figure}\par\noindent
% 
